Recent progress on correlated electron systems with strong spin-orbit coupling

Emergence of novel quantum ground states in correlated electron systems with strong spin-orbit coupling has been a recent subject of intensive studies. While it has been realized that spin-orbit coupling can provide non-trivial band topology in weakly interacting electron systems, as in topological insulators and semi-metals, the role of electron-electron interaction in strongly spin-orbit coupled systems has not been fully understood. The availability of new materials with significant electron correlation and strong spin-orbit coupling now makes such investigations possible. Many of these materials contain 5d or 4d transition metal elements; the prominent examples are iridium oxides or iridates. In this review, we succinctly discuss recent theoretical and experimental progress on this subject. After providing a brief overview, we focus on pyrochlore iridates and three-dimensional honeycomb iridates. In pyrochlore iridates, we discuss the quantum criticality of the bulk and surface states, and the relevance of the surface/boundary states in a number of topological and magnetic ground states, both in the bulk and thin film configurations. Experimental signatures of these boundary and bulk states are discussed. Domain wall formation and strongly-direction-dependent magneto-transport are also discussed. Regarding the three-dimensional honeycomb iridates, we consider possible quantum spin liquid phases and unusual magnetic orders in theoretical models with strongly bond-dependent interactions. These theoretical ideas and results are discussed in light of recent resonant X-ray scattering experiments on three-dimensional honeycomb iridates. We also contrast these results with the situation in two-dimensional honeycomb iridates. We conclude with the outlook on other related systems.

==> commands.tex <==
\newcommand{\twod}{$2$D}
\newcommand{\nairo}{Na${}_{2}$IrO${}_{3}$}
\newcommand{\aliiro}{$\alpha$-Li${}_{2}$IrO${}_{3}$}
\newcommand{\bliiro}{$\beta$-Li${}_{2}$IrO${}_{3}$}
\newcommand{\gliiro}{$\gamma$-Li${}_{2}$IrO${}_{3}$}
\newcommand{\liiro}{Li${}_{2}$IrO${}_{3}$}
\newcommand{\airo}{$A_{2}$IrO${}_{3}$}
\newcommand{\alirho}{$\alpha$-Li${}_{2}$RhO${}_{3}$}
\newcommand{\rucl}{RuCl$_3$}
\newcommand{\ttg}{$t_{2g}$}
\newcommand{\soc}{SOC}
\newcommand{\ve}[1]{\vec{#1}}
\newcommand{\liirotitle}{$\boldmath{\beta}\text{-Li}{}_{\boldmath{2}}\text{IrO}{}_{\boldmath{3}}$}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\ir}{$\text{Ir}^{4+}$}
\newcommand{\jhalf}{$j_{\text{eff}}=1/2$}
\newcommand{\jhalftitle}{$\boldmath{j_{\text{eff}}=1/2}$}
\newcommand{\jthreehalf}{$j_{\text{eff}}=3/2$}
\newcommand{\hhc}{hyper-honeycomb}
\newcommand{\harzero}{$\mathcal{H}\text{--}0$}
\newcommand{\har}{$\mathcal{H}\text{--}1$}
\newcommand{\xybond}{$X/Y$}
\newcommand{\zbond}{$Z$}
\newcommand{\Bzbond}{$Z_2$}
\newcommand{\NBzbond}{$Z_1$}
\newcommand{\jkg}{$JK\Gamma$}
\newcommand{\avg}[1]{\langle #1 \rangle}
\newcommand{\vhat}[1]{\vec{\hat{#1}}}
\newcommand{\uij}[2]{u^{#1}_{#2}}
\newcommand{\sutwo}{$SU(2)$}

\newcommand{\note}[1]{\textcolor{red}{#1}}
